V-RECS, a Low-Cost LLM4VIS Recommender with Explanations, Captioning and Suggestions

NL2VIS (natural language to visualization) is a promising and recent research area that involves interpreting natural language queries and translating them into visualizations that accurately represent the underlying data. As we navigate the era of big data, NL2VIS holds considerable application potential since it greatly facilitates data exploration by non-expert users. Following the increasingly widespread usage of generative AI in NL2VIS applications, in this paper we present V-RECS, the first LLM-based Visual Recommender augmented with explanations(E), captioning(C), and suggestions(S) for further data exploration. V-RECS' visualization narratives facilitate both response verification and data exploration by non-expert users. Furthermore, our proposed solution mitigates computational, controllability, and cost issues associated with using powerful LLMs by leveraging a methodology to effectively fine-tune small models. To generate insightful visualization narratives, we use Chain-of-Thoughts (CoT), a prompt engineering technique to help LLM identify and generate the logical steps to produce a correct answer. Since CoT is reported to perform poorly with small LLMs, we adopted a strategy in which a large LLM (GPT-4), acting as a Teacher, generates CoT-based instructions to fine-tune a small model, Llama-2-7B, which plays the role of a Student. Extensive experiments-based on a framework for the quantitative evaluation of AI-based visualizations and on manual assessment by a group of participants-show that V-RECS achieves performance scores comparable to GPT-4, at a much lower cost. The efficacy of the V-RECS teacher-student paradigm is also demonstrated by the fact that the un-tuned Llama fails to perform the task in the vast majority of test cases. We release V-RECS for the visualization community to assist visualization designers throughout the entire visualization generation process.

==> sections/conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}


==> sections/introduction.tex <==

\section{Introduction} \label{sec:introduction}
AI and Big Data development has reshaped how companies make decisions in recent years. A more data-driven approach has become increasingly crucial for companies to make more informed decisions, from big corporations to small and medium enterprises \cite{tawil2023trends}.
From marketing \cite{saura2023digital} to business intelligence, the data-centric strategy represents a terrific opportunity to keep up with a specific field's evolution and discover patterns that otherwise would be hidden.  
Notwithstanding, this introduces new challenges and complexity. The data analysis and transformation into actionable insights demand specific domain experts and economic resources. Often, especially for SMEs, these factors represent challenging aspects due to the need for more financial resources to recruit these specialized profiles. Furthermore, the supply of these specialized data scientists often falls short of meeting the burgeoning needs of the industry\footnote{\url{https://shorturl.at/ePUXY}}.

Visualization Recommendation Systems  (VRSs) try to fill the gap between non-expert users and data analysis \cite{podo2024agnostic} by providing automatic tools to support visual discovery from data across different sectors and applications. 
Many contributions have been developed in this field  (among others, \cite{hu2019vizml, luo2018deepeye, roth1994interactive, mackinlay1986automating}), some of which gained widespread adoption in well-known tools such as Tableau\footnote{\url{www.tableau.com}, which integrates a functionality named Suggest Me \cite{mackinlay2007show}}. To date,  state-of-the-art VRSs do not achieve full automation, relying on built-in knowledge (such as perceptual rules) or user input to guide the system in generating visualizations.
%, for example by entering natural language queries. This latter category of VRS is referred to in the literature as NL2VIS (Natural Language to Visualization). Many NL2VIS solutions rely on classic NLP (Natural Language Processing) or rule-based techniques \cite{setlur2016eviza, gao2015datatone, manning2014stanford} to translate the user's query, called Natural Language Query (NLQ), into insightful visualizations. \textcolor{red}{However,  reliance on these techniques poses a significant limitation, as it constrains users to adhere to specific formats (such as the need to clearly specify in the NLQ the type of chart and the variables to be plotted on the axes), thereby restricting the flexibility of expression in their queries. Furthermore, these approaches struggle to manage ambiguous texts, failing to produce a consistent and insightful visualization in many cases. } \textcolor{red}{PV: questa frase non piace ad un revisore}
%\textcolor{red}{Proposta: } 
%To date,  state-of-the-art VRSs do not achieve full automation, relying on built-in knowledge (such as perceptual rules) or user input to guide the system to generate visualizations, for example by entering natural language queries. c
Although fully automated systems may lack the flexibility for detailed customization that expert users might require, they %could also offer significant advantages:
can also help overcome many limitations of current approaches: 
\begin{itemize}
    \item Human visual perception (even when limited to chart interpretation) involves multiple processes, including color perception, pattern recognition, gestalt principles (proximity, similarity..), cognitive load, and more. Each of these processes is complex on its own, and capturing their interactions in a comprehensive set of rules is extremely challenging. Furthermore, rule-based approaches require manual updates to accommodate new scenarios. In contrast,  machine learning models can learn patterns, user preferences, and emerging trends, and adapt to new ones without needing explicit reprogramming.
    \item By integrating user specifications, VRSs may become more responsive and aligned with individual user preferences. On the other hand, this interaction implies knowledgeable users.  Users without a background in data analysis or visualization may find it challenging to provide the right query, indicate the right type of chart, or accurately interpret the data. 
\end{itemize}
%often lack the flexibility for detailed customization that expert users might require.

To address the first challenge, recent advancements in deep learning have enabled visual recommender systems to automatically learn perceptual rules from data/visualization pairs (see \cite{podo2024agnostic} for a recent survey).
In parallel, NL2Vis (Natural Language to Visualization) systems are being developed to simplify the interaction of non-expert users with complex data, by enabling them to generate visualizations through natural language queries (NLQ).  
Many NL2VIS solutions rely on classic NLP (Natural Language Processing) or rule-based techniques~\cite{setlur2016eviza, gao2015datatone, manning2014stanford} to translate the user's NLQ into insightful visualizations. However, reliance on these techniques poses a significant limitation, as it constrains users to adhere to specific formats (such as the need to clearly specify in the NLQ the type of chart and the variables to be plotted on the axes), thereby restricting the flexibility of expression in their queries. Furthermore, these approaches struggle to manage ambiguous texts, failing to produce a consistent and insightful visualization in many cases. To give an example, the system presented by Luo et al. \cite{luo2021natural}, despite its advanced Transformer-based architecture, still shows limitations in fully understanding and processing grammatically complex and/or semantically ambiguous sentences, as the authors point out.


A further significant step forward in the automation of visual recommender systems is represented by LLM4VIS (Large Language Models for Visualization) \cite{wang2023llm4vis}. By leveraging LLM technology in conjunction with advanced visualization techniques, LLM4VIS allows it to query data sources and translate them into visualizations that accurately represent the underlying data, showing advanced capabilities in understanding and processing complex natural language instructions.  
%systems can enhance the ability to understand, generate, and recommend visual content based on textual descriptions and data.
%Following the disruptive use of generative artificial intelligence across application domains, LLM4VIS (Large Language Model for Visualizations) \cite{wang2023llm4vis} is becoming one of the most promising research areas to advance existing NL2VIS approaches.
%, greatly improving the degree of free text in  NLQs.
%LLM4VIS aims to use cutting-edge LLM technology to query data sources using only natural language queries and translate them into visualizations that accurately represent the underlying data. 
It represents a promising direction in data visualization, offering significant advantages in terms of simplicity of user interaction, scalability, and ability to handle complex queries. However, even for these systems, many challenges remain open: 
\begin{itemize}
\item \textit{Interpretability and Trust:} Although LLM like Llama \cite{touvron2023llama} or GPT \cite{openai_gpt4}, have shown a more advanced semantic understanding of free text \cite{cheng2024exploring},
%In this direction, some approaches have already been proposed, such as Codeinterperter by OpenAI \cite{li2023prompting} or PandasAI, which enhance well-known libraries by involving LLM to query and navigate the data. PV: non si capisce esattamente "in this direction" e dunque lo ho commentato.
they suffer from the lack of interpretability of the model's responses \cite{wang2023deciphering} and hallucinations \cite{jha2023dehallucinating}. 
\item \textit{Controllability and cost:} ``Large'' LLM, those involving computationally intensive and expensive architectures containing billions, and recently trillions\footnote{as postulated by several sources, among which \url{https://the-decoder.com/gpt-4-has-a-trillion-parameters/} } of parameters, also have other contraindications, such as the lack of controllability \cite{controllability} and the high computational cost\footnote{in \url{https://shorturl.at/puz24} -among other published experiments - it is shown that Llama 2 obtains similar performance to GPT-4 for a fraction of the cost on a number of tasks}, hindering their large-scale adoption in applications.  In particular, controllability has a notable, and often neglected,  impact on applications: if a certain model is based on the adaptation of a proprietary LLM, such as GPT, the evolution of the original LLM\footnote{For example, there are notable differences between GPT-3 and GPT-4.} could significantly impact the adapted model. This means that developers of a model based on a proprietary LLM do not have full control of their system.

\item \textit{Adaptability and Verifiability:} Finally, although LLMs have proven great capabilities on tasks like text, images, or code generation, it has been observed that they are much less proficient on other tasks, such as data visualization and analysis. In this regard, Podo et al.~\cite{podo2024vi} observed how, even though GPT-3.5-turbo can already perform data visualization tasks, it still produces a high rate of errors and poses a problem of response verification, especially when the user is not sufficiently expert to evaluate the result. Unlike text and images, which can be easily verified by any user, or code, which can be verified by compiling and then validating the expected output, evaluating the quality of a recommended visualization is more challenging. If users do not know what to expect, or they are not domain experts, they may perceive the model's output as accurate, even when incorrect. 
\end{itemize}
To advance the field of automated visualization generation while addressing the challenges associated with generative AI-based solutions, in this paper we propose V-RECS, a LLM-based Visualization Recommender enhanced with three types of \textit{narratives }: Explanations (E), Captioning (C), and Suggestions for further data exploration (S). While E and C mitigate the problem of response verification,  S supports non-expert users to further explore the available data. The generated model,  based on a fine-tuned ``small'' LLM, Llama-2-7B, also mitigates cost and controllability issues\footnote{Llama-2-7B has seven billion parameters, while, e.g., GPT-4 has one trillion. Furthermore, Llama-2-7B is available free of charge for research and commercial use; in contrast, GPT-n models are proprietary, and their inner workings are hidden from the public \url{https://shorturl.at/bdoOZ}}.  

V-RECS' training methodology is based on Chain of Thoughts (CoT), a strategy to instruct a large LLM  to break down its responses into reasoning steps~\cite{wei2022chain}. Since CoT has been shown not to work well with small LLM~\cite{wang2023llm4vis}, we adopt a teacher-student paradigm in which GPT-4, the teacher, is asked to enrich with visualization narratives an existing dataset of users' queries and corresponding charts, leveraging the CoT strategy. Next, the enriched dataset is used to fine-tune a small open-source LLM, Llama-2-7B, to perform visualization recommendations along with producing textual narratives to explain and further explore the input data. 
%V-RECS is a pioneering research endeavor that aims to explore and showcase the application of LLM4VIS, \textcolor{red}{da qui in poi va cambiato tutto} combining the strength of LLMs with well-proofed visualization rules in literature. Unlike existing approaches outlined in the literature \cite{chen2022nl2interface, maddigan2023chat2vis} that involve prompt engineering techniques or Codeinterpreter by OpenAI \cite{li2023prompting} that wraps the model into a python environment to run the code, NewtonLLM tries to be the first data-scientist LLM, processing the NQL without any additional input or environment. The strategy behind NewtonLLM involves harnessing the LLM fine-tuning framework introduced by \cite{ho2022large} alongside the VegaZero grammar proposed by \cite{ncnet}. Additionally, NewtonLLM presents a novel strategy for integrating visualization rules into the LLM reinforcement learning process.
V-RECS exploits the synergies between LLM and the visualization field, to improve the generation of insightful visual representations from data, while ensuring that the user has full control over the reliability of what is suggested by the Visual Recommender.
The main contributions of this work are:
\begin{itemize}
    \item V-RECS, the first LLM fine-tuned for the visualization field that performs fully automated visualization recommendation along with the production of insightful visualization narratives;
     \item Low-cost and controllable solution: V-RECS is based on fine-tuning the open source Llama-2-7B, which was estimated to be 100 times less expensive than GPT-4, along with the other previously summarized advantages of low-parameter Open-AI models \footnote{amongst the many studies, see e.g.,\url{https://tinyurl.com/56kpjd7r}}. Despite leveraging a small LLM, V-RECS achieves performances comparable to GPT-4, as shown in Section \ref{sec:evaluation}. 
    \item LLM4VIS methodology: we present an end-to-end solution for LLM4VIS, contributing a novel approach leveraging contributions from generative artificial intelligence, explainable machine learning, and the visualization field.   
    \item A comprehensive comparative quantitative and qualitative evaluation experiment,  to study how the proposed V-RECS model and GPT-4 perform the visualization task. 
\end{itemize}
We release V-RECS for the visualization community on a GitHub repository\footnote{\url{https://github.com/lucapodo/V-RECS.git}}.

The paper is organized as follows: in Section \ref{sec:LLMs} we summarize the main concepts of LLM. Section \ref{sec:related_works} is dedicated to the state-of-the-art in NL2VIS and LLM4VIS. Section \ref{sec:problem_formulation} presents a formal description of the LLM4VIS problem. Section \ref{sec:method} describes the proposed V-RECS model and the LLM-based methodology to develop it.  Section \ref{sec:evaluation} reports the results of quantitative and qualitative evaluation activities. Finally, we present a discussion and our concluding remarks in Section \ref{sec:discussion}.

==> sections/open_challenges.tex <==
Thanks to recent developments in deep learning and NLP, NL2VIS has seen an increased interest from researchers and industries working in this field. Although the domain has already been addressed in the literature with classical NLP or rule-based techniques, advanced deep learning approaches such as transformers or LLM have opened up new scenarios that make this field still unexplored and in its infancy, as highlighted in \cite{maddigan2023chat2vis}. For this reason, the area is constrained by several open challenges. Some of the most prominent challenges we have identified are:

\begin{itemize}
  \item \textbf{LLM complexity}. While these models enhance the semantic understanding of texts, they also introduce significant complexity. Currently, the techniques that allow these models to be modified and adapted to specific tasks are mainly those of few-shot learning or fine-tuning \cite{wang2020generalizing}, as it is currently difficult to train an LLM model from scratch. This leads to a substantial dependence on the solutions in the literature on the language models made available by the big players such as OpenAI, creating problems of data privacy, fairness, and reliability that have recently been the subject of intense public debate.
  \item \textbf{lack of a standard visualization grammar} for NL2VIS task. The study of specific and standard grammar is crucial to building up novel approaches that can face optimizing the translation problem. \textcolor{blue}{Io qui allungherei, introducendo ad es i limiti dei vari vega-x e di altri approcci. Sennò è poco sostanziata, la critica.}
  \item \textbf{lack of benchmarks}. The only valuable contribution is nvBench \cite{luo2021empowering}, whose primary constraint regards the bias introduced during the synthetic generation process  
  \item \textbf{NLQs variation}. The input is a free text form that allows the user to specify a visualization using different NLQ specifications, e.g., draw a line chart or show me the time trend. Such NLQs are semantically identical and ask for the same visualization; for this reason, the NLQ variation represents a semantic interpretation challenge \textcolor{blue}{cioè vuoi dire: nel dataset hai coppie query-specifica, ma a query  sintatticamente diverse ma semanticamente simili o uguali può corrispondere la stessa specifica, e NvBench non include queste varianti, quindi un sistema NL2Vis dovrenbbe essere in grado di estrapolarle?}. A model should be able to recognize the two inputs as semantically correlated and proposes the same visualization for both. This requires broad knowledge and prior information about how the users pose different NLQ specifications \textcolor{blue}{se la butti sul prior knowledge non ne esci, qui semplicemente è necessario che il sistema sia automaticamente in grado di mappare frasi diverse in una rappresentazione semantica ``profonds'' che ne catturi la similarità}.
  \item \textbf{NLQs ambiguity} relates to the model's difficulty in choosing the proper dataset columns when they are not explicitly expressed in the NLQ. For example, consider the dataset \textit{sex} and \textit{age} column names. The problem arises when the user intends to study the age distribution among the sexes asking \textit{``Show me the different ages per group''}. In this case, the user correlated the term ``group'' to the column ``sex'' but did not write the column name explicitly.
  \item \textbf{lack of evaluation metrics}. The only metric available is the accuracy against the different visualization specifications described in section [ref]. Evaluation of visualization is a complex task involving several human-related factors, such as perceptual insightfulness, that makes it difficult to measure the correctness of a result quantitatively. Without metrics that simulate human perceptual behavior, reliance solely on accuracy metrics can be problematic. Weaknesses can arise if the dataset is not well-structured. \textcolor{blue}{anche qui fai esempi e magari metti figure}
  \item \textbf{User intreaction NL2VIS approaches}. All the approaches surveyed in this paper implement solutions where the user interaction is confined to asking the visualization. None of them explore how to allow the user to refine the visualizations once generated. This is a crucial task to improve these kinds of solutions.While feedback requests are generally discouraged in applications targeting general users due to their potential to bore users, this particular case caters to professionals seeking efficient data analysis support that facilitates quick insights. Hence, it is reasonable to assume that these users are willing to iteratively refine their requests in multiple steps.
\end{itemize}
